Arbitrary Lagrangian--Eulerian finite element method for lipid membranes

An arbitrary Lagrangian--Eulerian finite element method and numerical implementation for curved and deforming lipid membranes is presented here. The membrane surface is endowed with a mesh whose in-plane motion need not depend on the in-plane flow of lipids. Instead, in-plane mesh dynamics can be specified arbitrarily. A new class of mesh motions is introduced, where the mesh velocity satisfies the dynamical equations of a user-specified two-dimensional material. A Lagrange multiplier constrains the out-of-plane membrane and mesh velocities to be equal, such that the mesh and material always overlap. An associated numerical inf--sup instability ensues, and is removed by adapting established techniques in the finite element analysis of fluids. In our implementation, the aforementioned Lagrange multiplier is projected onto a discontinuous space of piecewise linear functions. The new mesh motion is compared to established Lagrangian and Eulerian formulations by investigating a preeminent numerical benchmark of biological significance: the pulling of a membrane tether from a flat patch, and its subsequent lateral translation.

==> abstract.tex <==
An arbitrary Lagrangian--Eulerian finite element method and numerical
implementation for curved and deforming lipid membranes is presented here.
The membrane surface is endowed with a mesh whose in-plane motion need not
depend on the in-plane flow of lipids.
Instead, in-plane mesh dynamics can be specified arbitrarily.
A new class of mesh motions is introduced, where the mesh velocity satisfies
the dynamical equations of a user-specified two-dimensional material.
A Lagrange multiplier constrains the out-of-plane membrane and mesh velocities
to be equal, such that the mesh and material always overlap.
An associated numerical inf--sup instability ensues, and is removed by adapting
established techniques in the finite element analysis of fluids.
In our implementation, the aforementioned Lagrange multiplier is projected onto
a discontinuous space of piecewise linear functions.
The new mesh motion is compared to established Lagrangian and Eulerian
formulations by investigating a preeminent numerical benchmark of biological
significance: the pulling of a membrane tether from a flat patch, and its
subsequent lateral translation.



%Biological membranes are unique two-dimensional materials in which lipids flow in-plane as a Newtonian fluid, while the entire membrane bends out-of-plane as an elastic sheet. Though the dynamical equations governing lipid membranes are known, they are analytically intractable: membrane dynamics are highly nonlinear and involve spatial derivatives on a surface which is itself arbitrarily curved and deforming over time. The challenges in analytically solving the membrane equations extend to their numerical solution as well: standard computational techniques from fluid and solid mechanics cannot model a two-dimensional material with arbitrarily large shape deformations, in-plane flows, and out-of-plane elasticity. We address this issue by developing an arbitrary Lagrangian–Eulerian (ALE) finite element method for lipid membranes. The membrane surface is endowed with a mesh whose in-plane motion can be specified independently of the material velocity; the out-of-plane mesh motion is required to be Lagrangian such that the mesh and material always overlap. A new in-plane mesh motion is implemented, in which the mesh evolves according to the dynamical equations governing a two-dimensional area-compressible viscoelastic fluid film. Our scheme is used to simulate the long-time dynamics of unstable lipid membranes in biologically-relevant scenarios, including the non-axisymmetric buckling and wrinkling of an membrane tube. The tension propagation in situations where tethers are pulled from membrane sheets and cylinders is also quantified. Finally, we show how to extend our numerical implementation to describe surfaces with more complex rheology.


==> cc-greek-letters.tex <==



%% tilde Greek letters
\newcommand{\tillambda}{\tilde{\lambda}}
\newcommand{\tilpsi}{\tilde{\psi}}


%% bar Greek letters
\newcommand{\barpsi}{\bar{\psi}}


%% check Greek indices
\newcommand{\calpha}{{\check{\alpha}}}
\newcommand{\cbeta}{{\check{\beta}}}
\newcommand{\cgamma}{{\mkern3mu\check{\mkern-3mu\gamma}}}
\newcommand{\cdelta}{{\check{\delta}}}
\newcommand{\ceta}{{\check{\eta}}}
\newcommand{\clambda}{{\check{\lambda}}}
\newcommand{\cmu}{{\check{\mu}}}
\newcommand{\cnu}{{\check{\nu}}}
\newcommand{\crho}{{\check{\rho}}}
\newcommand{\csigma}{{\check{\sigma}}}


%% hat Greek indices
\newcommand{\halpha}{{\hat{\alpha}}}
\newcommand{\hbeta}{{\hat{\beta}}}
\newcommand{\hgamma}{{\hat{\gamma}}}
\newcommand{\hdelta}{{\hat{\delta}}}
\newcommand{\heta}{{\hat{\eta}}}
\newcommand{\hlambda}{{\hat{\lambda}}}
\newcommand{\hmu}{{\hat{\mu}}}
\newcommand{\hnu}{{\hat{\nu}}}
\newcommand{\hrho}{{\hat{\rho}}}
\newcommand{\hsigma}{{\hat{\sigma}}}


%% bold Greek letters
\newcommand{\bmalpha}{\bm{\alpha}}
\newcommand{\bmbeta}{\bm{\beta}}
\newcommand{\bmchi}{\bm{\chi}}
\newcommand{\bmvarepsilon}{\pmb{\bm{\varepsilon}}}
\newcommand{\bmkappa}{\bm{\kappa}}
\newcommand{\bmlambda}{\bm{\lambda}}
\newcommand{\bmmu}{\bm{\mu}}
\newcommand{\bmnu}{\bm{\nu}}
\newcommand{\bmsigma}{\bm{\sigma}}
\newcommand{\bmtau}{\bm{\tau}}


%% italicized Greek letters (upper case)
\newcommand{\itDelta}{\mathit{\Delta}}
\newcommand{\itGamma}{\mathit{\Gamma}}
\newcommand{\itLambda}{\mathit{\Lambda}}
\newcommand{\itOmega}{\mathit{\Omega}}
\newcommand{\itPhi}{\mathit{\Phi}}
\newcommand{\itSigma}{\mathit{\Sigma}}





==> cc-roman-letters.tex <==



%% bold Roman letters (lower case)
\newcommand{\bma}{\bm{a}}
\newcommand{\bmb}{\bm{b}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bmd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmg}{\bm{g}}
\newcommand{\bmh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmk}{\bm{k}}
\newcommand{\bml}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmo}{\bm{o}}
\newcommand{\bmp}{\bm{p}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bms}{\bm{s}}
\newcommand{\bmt}{\bm{t}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmy}{\bm{y}}
\newcommand{\bmz}{\bm{z}}


%% bold Roman letters (upper case)
\newcommand{\bmA}{\bm{A}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmG}{\bm{G}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmN}{\bm{N}}
\newcommand{\bmO}{\bm{O}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmT}{\bm{T}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmX}{{\bm{X}}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmZ}{\bm{Z}}


%% bold upright Roman letters (upper case)
\newcommand{\mathbfA}{\mathbf{A}}
\newcommand{\mathbfB}{\mathbf{B}}
\newcommand{\mathbfC}{\mathbf{C}}
\newcommand{\mathbfD}{\mathbf{D}}
\newcommand{\mathbfE}{\mathbf{E}}
\newcommand{\mathbfF}{\mathbf{F}}
\newcommand{\mathbfG}{\mathbf{G}}
\newcommand{\mathbfH}{\mathbf{H}}
\newcommand{\mathbfI}{\mathbf{I}}
\newcommand{\mathbfJ}{\mathbf{J}}
\newcommand{\mathbfK}{\mathbf{K}}
\newcommand{\mathbfL}{\mathbf{L}}
\newcommand{\mathbfM}{\mathbf{M}}
\newcommand{\mathbfN}{\mathbf{N}}
\newcommand{\mathbfO}{\mathbf{O}}
\newcommand{\mathbfP}{\mathbf{P}}
\newcommand{\mathbfQ}{\mathbf{Q}}
\newcommand{\mathbfR}{\mathbf{R}}
\newcommand{\mathbfS}{\mathbf{S}}
\newcommand{\mathbfT}{\mathbf{T}}
\newcommand{\mathbfU}{\mathbf{U}}
\newcommand{\mathbfV}{\mathbf{V}}
\newcommand{\mathbfW}{\mathbf{W}}
\newcommand{\mathbfX}{\mathbf{X}}
\newcommand{\mathbfY}{\mathbf{Y}}
\newcommand{\mathbfZ}{\mathbf{Z}}


%% bold upright Roman letters (lower case)
\newcommand{\mathbfa}{\mathbf{a}}
\newcommand{\mathbfb}{\mathbf{b}}
\newcommand{\mathbfc}{\mathbf{c}}
\newcommand{\mathbfd}{\mathbf{d}}
\newcommand{\mathbfe}{\mathbf{e}}
\newcommand{\mathbff}{\mathbf{f}}
\newcommand{\mathbfg}{\mathbf{g}}
\newcommand{\mathbfh}{\mathbf{h}}
\newcommand{\mathbfi}{\mathbf{i}}
\newcommand{\mathbfj}{\mathbf{j}}
\newcommand{\mathbfk}{\mathbf{k}}
\newcommand{\mathbfl}{\mathbf{l}}
\newcommand{\mathbfm}{\mathbf{m}}
\newcommand{\mathbfn}{\mathbf{n}}
\newcommand{\mathbfo}{\mathbf{o}}
\newcommand{\mathbfp}{\mathbf{p}}
\newcommand{\mathbfq}{\mathbf{q}}
\newcommand{\mathbfr}{\mathbf{r}}
\newcommand{\mathbfs}{\mathbf{s}}
\newcommand{\mathbft}{\mathbf{t}}
\newcommand{\mathbfu}{\mathbf{u}}
\newcommand{\mathbfv}{\mathbf{v}}
\newcommand{\mathbfw}{\mathbf{w}}
\newcommand{\mathbfx}{\mathbf{x}}
\newcommand{\mathbfy}{\mathbf{y}}
\newcommand{\mathbfz}{\mathbf{z}}


%% math calligraphy letters
\newcommand{\mca}{\mathcal{A}}
\newcommand{\mcb}{\mathcal{B}}
\newcommand{\mcc}{\mathcal{C}}
\newcommand{\mcd}{\mathcal{D}}
\newcommand{\mce}{\mathcal{E}}
\newcommand{\mcf}{\mathcal{F}}
\newcommand{\mcg}{\mathcal{G}}
\newcommand{\mch}{\mathcal{H}}
\newcommand{\mci}{\mathcal{I}}
\newcommand{\mcj}{\mathcal{J}}
\newcommand{\mck}{\mathcal{K}}
\newcommand{\mcl}{\mathcal{L}}
\newcommand{\mcm}{\mathcal{M}}
\newcommand{\mcn}{\mathcal{N}}
\newcommand{\mco}{\mathcal{O}}
\newcommand{\mcp}{\mathcal{P}}
\newcommand{\mcq}{\mathcal{Q}}
\newcommand{\mcr}{\mathcal{R}}
\newcommand{\mcs}{\mathcal{S}}
\newcommand{\mct}{\mathcal{T}}
\newcommand{\mcu}{\mathcal{U}}
\newcommand{\mcv}{\mathcal{V}}
\newcommand{\mcw}{\mathcal{W}}
\newcommand{\mcx}{\mathcal{X}}
\newcommand{\mcy}{\mathcal{Y}}
\newcommand{\mcz}{\mathcal{Z}}


%% math script letters
\newcommand{\sca}{{\mathscr{A}}}
\newcommand{\scb}{{\mathscr{B}}}
\newcommand{\scc}{{\mathscr{C}}}
\newcommand{\scd}{{\mathscr{D}}}
\newcommand{\sce}{{\mathscr{E}}}
\newcommand{\scf}{{\mathscr{F}}}
\newcommand{\scg}{{\mathscr{G}}}
\newcommand{\sch}{{\mathscr{H}}}
\newcommand{\sci}{{\mathscr{I}}}
\newcommand{\scj}{{\mathscr{J}}}
\newcommand{\sck}{{\mathscr{K}}}
\newcommand{\scl}{{\mathscr{L}}}
\newcommand{\scm}{{\mathscr{M}}}
\newcommand{\scn}{{\mathscr{N}}}
\newcommand{\sco}{{\mathscr{O}}}
\newcommand{\scp}{{\mathscr{P}}}
\newcommand{\scq}{{\mathscr{Q}}}
\newcommand{\scr}{{\mathscr{R}}}
\newcommand{\scs}{{\mathscr{S}}}
\newcommand{\sct}{{\mathscr{T}}}
\newcommand{\scu}{{\mathscr{U}}}
\newcommand{\scv}{{\mathscr{V}}}
\newcommand{\scw}{{\mathscr{W}}}
\newcommand{\scx}{{\mathscr{X}}}
\newcommand{\scy}{{\mathscr{Y}}}
\newcommand{\scz}{{\mathscr{Z}}}


% Roman math mode letters (lower case)
\newcommand{\ta}{{\mathrm{a}}}
\newcommand{\tb}{{\mathrm{b}}}
\newcommand{\tc}{{\mathrm{c}}}
\newcommand{\td}{{\mathrm{d}}}
\newcommand{\te}{{\mathrm{e}}}
\newcommand{\tf}{{\mathrm{f}}}
\newcommand{\tg}{{\mathrm{g}}}
\newcommand{\mh}{{\mathrm{h}}}
\newcommand{\ti}{{\mathrm{i}}}
\newcommand{\tj}{{\mathrm{j}}}
\newcommand{\tk}{{\mathrm{k}}}
\newcommand{\tl}{{\mathrm{l}}}
\newcommand{\tm}{{\mathrm{m}}}
\newcommand{\tn}{{\mathrm{n}}}
\newcommand{\mo}{{\mathrm{o}}}
\newcommand{\tp}{{\mathrm{p}}}
\newcommand{\tq}{{\mathrm{q}}}
\newcommand{\tr}{{\mathrm{r}}}
\newcommand{\ts}{{\mathrm{s}}}
\newcommand{\mt}{{\mathrm{t}}}
\newcommand{\tv}{{\mathrm{v}}}
\newcommand{\tw}{{\mathrm{w}}}
\newcommand{\tx}{{\mathrm{x}}}
\newcommand{\ty}{{\mathrm{y}}}
\newcommand{\tz}{{\mathrm{z}}}


% Roman math mode letters (upper case)
\newcommand{\tA}{{\mathrm{A}}}
\newcommand{\tB}{{\mathrm{B}}}
\newcommand{\tC}{{\mathrm{C}}}
\newcommand{\tD}{{\mathrm{D}}}
\newcommand{\tE}{{\mathrm{E}}}
\newcommand{\tF}{{\mathrm{F}}}
\newcommand{\tG}{{\mathrm{G}}}
\newcommand{\tH}{{\mathrm{H}}}
\newcommand{\tI}{{\mathrm{I}}}
\newcommand{\tJ}{{\mathrm{J}}}
\newcommand{\tK}{{\mathrm{K}}}
\newcommand{\tL}{{\mathrm{L}}}
\newcommand{\tM}{{\mathrm{M}}}
\newcommand{\tN}{{\mathrm{N}}}
\newcommand{\tO}{{\mathrm{O}}}
\newcommand{\tP}{{\mathrm{P}}}
\newcommand{\tQ}{{\mathrm{Q}}}
\newcommand{\tR}{{\mathrm{R}}}
\newcommand{\tS}{{\mathrm{S}}}
\newcommand{\tT}{{\mathrm{T}}}
\newcommand{\tU}{{\mathrm{U}}}
\newcommand{\tV}{{\mathrm{V}}}
\newcommand{\tW}{{\mathrm{W}}}
\newcommand{\tX}{{\mathrm{X}}}
\newcommand{\tY}{{\mathrm{Y}}}
\newcommand{\tZ}{{\mathrm{Z}}}


% tilde Roman letters (lower case)
\newcommand{\tila}{\tilde{a}}
\newcommand{\tilb}{\tilde{b}}
\newcommand{\tilc}{\tilde{c}}
\newcommand{\tild}{\tilde{d}}
\newcommand{\tile}{\tilde{e}}
\newcommand{\tilf}{\tilde{f}}
\newcommand{\tilg}{\tilde{g}}
\newcommand{\tilh}{\tilde{h}}
\newcommand{\tili}{\tilde{i}}
\newcommand{\tilj}{\tilde{j}}
\newcommand{\tilk}{\tilde{k}}
\newcommand{\tilm}{\tilde{m}}
\newcommand{\tiln}{\tilde{n}}
\newcommand{\tilo}{\tilde{o}}
\newcommand{\tilp}{\tilde{p}}
\newcommand{\tilq}{\tilde{q}}
\newcommand{\tilr}{\tilde{r}}
\newcommand{\tils}{\tilde{s}}
\newcommand{\tilt}{\tilde{t}}
\newcommand{\tilu}{\tilde{u}}
\newcommand{\tilv}{\tilde{v}}
\newcommand{\tilw}{\tilde{w}}
\newcommand{\tilx}{\tilde{x}}
\newcommand{\tily}{\tilde{y}}
\newcommand{\tilz}{\tilde{z}}


% tilde Roman letters (upper case)
\newcommand{\tilA}{\mkern5.5mu\tilde{\mkern-5.5mu A}}
\newcommand{\tilB}{\tilde{B}}
\newcommand{\tilC}{\tilde{C}}
\newcommand{\tilD}{\tilde{D}}
\newcommand{\tilE}{\tilde{E}}
\newcommand{\tilF}{\tilde{F}}
\newcommand{\tilG}{\tilde{G}}
\newcommand{\tilH}{\tilde{H}}
\newcommand{\tilI}{\tilde{I}}
\newcommand{\tilJ}{\tilde{J}}
\newcommand{\tilK}{\tilde{K}}
\newcommand{\tilL}{\tilde{L}}
\newcommand{\tilM}{\tilde{M}}
\newcommand{\tilN}{\tilde{N}}
\newcommand{\tilO}{\tilde{O}}
\newcommand{\tilP}{\tilde{P}}
\newcommand{\tilQ}{\tilde{Q}}
\newcommand{\tilR}{\tilde{R}}
\newcommand{\tilS}{\tilde{S}}
\newcommand{\tilT}{\tilde{T}}
\newcommand{\tilU}{\tilde{U}}
\newcommand{\tilV}{\tilde{V}}
\newcommand{\tilW}{\tilde{W}}
\newcommand{\tilX}{\tilde{X}}
\newcommand{\tilY}{\tilde{Y}}
\newcommand{\tilZ}{\tilde{Z}}


%% bar Roman letters (lower case)
\newcommand{\bara}{\bar{a}}
\newcommand{\barb}{\bar{b}}
\newcommand{\barc}{\bar{c}}
\newcommand{\bard}{\bar{d}}
\newcommand{\bare}{\bar{e}}
\newcommand{\barf}{\bar{f}}
\newcommand{\barg}{\bar{g}}
\newcommand{\barh}{\bar{h}}
\newcommand{\bari}{\bar{i}}
\newcommand{\barj}{\bar{j}}
\newcommand{\bark}{\bar{k}}
\newcommand{\barl}{\bar{l}}
\newcommand{\barm}{\bar{m}}
\newcommand{\barn}{\bar{n}}
%\newcommand{\baro}{\bar{o}}
\newcommand{\barp}{\bar{p}}
\newcommand{\barq}{\bar{q}}
\newcommand{\barr}{\bar{r}}
\newcommand{\bars}{\bar{s}}
\newcommand{\bart}{\mkern0.0mu\overline{\mkern-0.0mu t\mkern1.2mu}\mkern-1.2mu}
\newcommand{\baru}{\bar{u}}
\newcommand{\barv}{\bar{v}}
\newcommand{\barw}{\bar{w}}
\newcommand{\barx}{\bar{x}}
\newcommand{\bary}{\bar{y}}
\newcommand{\barz}{\bar{z}}


%% bar Roman letters (upper case)
\newcommand{\barA}{\bar{A}}
\newcommand{\barB}{\bar{B}}
\newcommand{\barC}{\bar{C}}
\newcommand{\barD}{\bar{D}}
\newcommand{\barE}{\bar{E}}
\newcommand{\barF}{\mkern4.5mu\overline{\mkern-4.5mu F \mkern-0.5mu}\mkern0.5mu}
\newcommand{\barG}{\bar{G}}
\newcommand{\barH}{\bar{H}}
\newcommand{\barI}{\bar{I}}
\newcommand{\barJ}{\bar{J}}
\newcommand{\barK}{\bar{K}}
\newcommand{\barL}{\bar{L}}
\newcommand{\barM}{\mkern4.5mu\overline{\mkern-4.5mu M \mkern-1.5mu}\mkern1.5mu}
\newcommand{\barN}{\bar{N}}
\newcommand{\barO}{\bar{O}}
\newcommand{\barP}{\bar{P}}
\newcommand{\barQ}{\bar{Q}}
\newcommand{\barR}{\bar{R}}
\newcommand{\barS}{\bar{S}}
\newcommand{\barT}{\bar{T}}
\newcommand{\barU}{\bar{U}}
\newcommand{\barV}{\bar{V}}
\newcommand{\barW}{\bar{W}}
\newcommand{\barX}{\bar{X}}
\newcommand{\barY}{\bar{Y}}
\newcommand{\barZ}{\bar{Z}}


% hat Roman letters (lower case)
\newcommand{\hata}{\hat{a}}
\newcommand{\hatb}{\hat{b}}
\newcommand{\hatc}{\hat{c}}
\newcommand{\hatd}{\hat{d}}
\newcommand{\hate}{\hat{e}}
\newcommand{\hatf}{\hat{f}}
\newcommand{\hatg}{\hat{g}}
\newcommand{\hath}{\hat{h}}
\newcommand{\hati}{\hat{i}}
\newcommand{\hatj}{\hat{j}}
\newcommand{\hatk}{\hat{k}}
\newcommand{\hatl}{\hat{l}}
\newcommand{\hatm}{\hat{m}}
\newcommand{\hatn}{\hat{n}}
\newcommand{\hato}{\hat{o}}
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatq}{\hat{q}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hats}{\hat{s}}
\newcommand{\hatt}{\hat{t}}
\newcommand{\hatu}{\hat{u}}
\newcommand{\hatv}{\hat{v}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\hatx}{\hat{x}}
\newcommand{\haty}{\hat{y}}
\newcommand{\hatz}{\hat{z}}


% hat Roman letters (upper case)
\newcommand{\hatA}{\mkern7.0mu\hat{\mkern-7.0mu A}}



==> custom-commands.tex <==

% highlighting
\newcommand{\code}[1]{\textcolor{red}{#1}}

% define colors
\definecolor{myCyan}{rgb}{0.0, 0.47, 0.75}  \colorlet{myBlue}{blue!70!green}
\colorlet{myOrange}{red!60!yellow}          \colorlet{myRed}{orange!40!purple}
\colorlet{myGreen}{green!70!blue}           \colorlet{myPurple}{red!60!blue}
\colorlet{myDarkCyan}{myPurple!15!myCyan}

% reviewer edits
%\newcommand{\reva}[1]{\textcolor{myGreen}{#1}}
%\newcommand{\revb}[1]{\textcolor{magenta}{#1}}
%\newcommand{\revc}[1]{\textcolor{myDarkCyan}{#1}}
%\newcommand{\both}[1]{\textcolor{myOrange}{#1}}			% add from both reviewers
%\newcommand{\remove}[1]{\textcolor{gray}{\sout{#1}}}	% material to remove
%\newcommand{\remeq}[1]{\textcolor{gray}{#1}}			% equation to remove


% spacing
\newcommand{\mk}{\mkern1mu}
\newcommand{\mkn}{\mkern-1mu}

% operators
\newcommand{\bmcdot}{\bm{\cdot}}
\newcommand{\Deltas}{\Delta_\ts}
\newcommand{\jj}[1]{\left\llbracket \mk #1 \mk \right\rrbracket}
\newcommand{\mathbfInen}{[ \mathbfI^\nen_{(3)} ]}
\newcommand{\pdp}{(\, \bmcdot \,)}

% new square root definition
% from https://en.wikibooks.org/wiki/LaTeX/Mathematics#Roots
\def\sqrtl{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\sqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.2\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}

% total and partial derivatives
\newcommand{\dd}[2]{\dfrac{\td \mk {#1}}{\td \mk {#2}}}
\newcommand{\ddt}[2]{\dfrac{\td^2 \mk {#1}}{\td \mk {#2}^2}}
\newcommand{\ddth}[2]{\dfrac{\td^3 \mk {#1}}{\td \mk {#2}^3}}
\newcommand{\pp}[2]{\dfrac{\partial \mk {#1}}{\partial \mk {#2}}}


\newcommand{\ale}{\texttt{ALE}}
\newcommand{\alev}{\texttt{ALE-v}}
\newcommand{\alevb}{\texttt{ALE-vb}}
\newcommand{\eul}{\texttt{EUL}}
\newcommand{\julia}{\texttt{Julia}}
\newcommand{\lag}{\texttt{LAG}}
\newcommand{\memalefem}{\texttt{MembraneAleFem.jl}}


% 
\newcommand{\bmej}{\bme_j}
\newcommand{\bmex}{\bme_x}
\newcommand{\bmey}{\bme_y}
\newcommand{\bmez}{\bme_z}
\newcommand{\bmer}{\bme_r}
\newcommand{\bmetheta}{\bme^{}_\theta}

%
\newcommand{\bmaa}{\bma^{}_\calpha}
\newcommand{\bmab}{\bma^{}_\cbeta}
\newcommand{\bmTa}{\bmT^\calpha}
\newcommand{\bmTam}{\bmTa_\tm}
\newcommand{\bmTamv}{\bmTa_{\tm, \mk \texttt{v}}}
\newcommand{\bmTamvb}{\bmTa_{\tm, \mk \texttt{vb}}}

\newcommand{\auabl}{a^{\calpha} {\hspace{-1.0pt}}^\text{\raisebox{-1ex}{$\cbeta$}}}
\newcommand{\piab}{\pi^{\calpha \cbeta}}
\newcommand{\piabm}{\piab_\tm}
\newcommand{\sigmaab}{\sigma^{\calpha \cbeta}}
\newcommand{\sigmaabl}{\sigma^{\calpha} {\hspace{-1.0pt}}^\text{\raisebox{-1ex}{$\cbeta$}}}
\newcommand{\sigmaabm}{\sigmaab_\tm}
\newcommand{\sigmaabmv}{\sigmaab_{\tm, \mk \texttt{v}}}
\newcommand{\sigmaabmvb}{\sigmaab_{\tm, \mk \texttt{vb}}}
\newcommand{\Mm}{M^{\tm}}
\newcommand{\Mab}{M^{\calpha \cbeta}}
\newcommand{\Mabm}{\Mab_\tm}
\newcommand{\Mabmv}{\Mab_{\tm, \mk \texttt{v}}}
\newcommand{\Mabmvb}{\Mab_{\tm, \mk \texttt{vb}}}


% membrane material properties
\newcommand{\kb}{k_\tb}
\newcommand{\kg}{k_\tg}

\newcommand{\kbm}{k^\tm_\tb}
\newcommand{\kgm}{k^\tm_\tg}

\newcommand{\mubar}{\bar{\mu}}
\newcommand{\lambdabar}{\bar{\lambda}}

% membrane tube/cylinder
\newcommand{\rc}{r_{\! \tc}}
\newcommand{\vc}{v_{\tc}}

% boundary conditions
\newcommand{\Fj}{F_{\! j}}
\newcommand{\Fmj}{F^\tm_{\! j}}
\newcommand{\bmFm}{\bmF^\tm}
\newcommand{\bmFmv}{\bmFm_{\texttt{v}}}
\newcommand{\bmFmvb}{\bmFm_{\texttt{vb}}}
\newcommand{\barFj}{\barF_{\! j}}
\newcommand{\barFjm}{\barF^\tm_{\! j}}
\newcommand{\bmfbar}{\bm{\bar{f}}}
\newcommand{\bmFbar}{\bm{\bar{F}}}
\newcommand{\GammaFmj}{\Gamma_{\!\! F}^{\tm \mk j}}
\newcommand{\GammaFj}{\Gamma_{\!\! F}^{\mk j}}
\newcommand{\GammaM}{\Gamma_{\! M}}
\newcommand{\Gamman}{\Gamma_{\! n}}
\newcommand{\Gammavmj}{\Gamma_{\! v}^{\tm \mk j}}
\newcommand{\Gammavj}{\Gamma_{\! v}^{\mk j}}
\newcommand{\vmj}{v^{\tm}_{\mkn j}}
\newcommand{\vj}{v^{}_{\mkn j}}
\newcommand{\barvj}{\barv^{}_{\mkn j}}
\newcommand{\barvjm}{\barv^{\tm}_{\mkn j}}

% simulation parameters
\newcommand{\ttf}{t^{}_\tf}
\newcommand{\ttm}{t^{}_\tm}
\newcommand{\ttM}{t^{}_\tM}
\newcommand{\barMf}{\barM_{\! \tf}}
\newcommand{\alpham}{\alpha^{\tm}}
\newcommand{\alphamE}{\alpha_{\tm}^{\texttt{E}}}
\newcommand{\alphamV}{\alpha_{\tm}^{\texttt{V}}}

% Dohrmann--Bochev
\newcommand{\alphaDB}{\alpha^{\text{DB}}}
\newcommand{\brlambda}{\breve{\lambda}}
\newcommand{\brL}{\mkern1.5mu\breve{\mkern-1.5mu L}}
\newcommand{\brN}{\mkern3.0mu\breve{\mkern-3.0mu N}}
\newcommand{\brNe}[1]{\mkern-4.5mu\breve{\mkern4.5mu N^e_{#1}}}
\newcommand{\brNek}{\brNe{k}}
\newcommand{\brp}{\breve{p}}
\newcommand{\brpm}{\brp^{\mk \tm}}
\newcommand{\brpme}{\brp^{\mk \tm, e}}

% initial conditions
\newcommand{\lambdaz}{\lambda_0}
\newcommand{\bmxz}{\bmx^{}_0}

% stability analysis
\newcommand{\omegai}{\omega^{(i)}}
\newcommand{\omegar}{\omega^{(r)}}
\newcommand{\Omegai}{\Omega^{(i)}}
\newcommand{\Omegar}{\Omega^{(r)}}


% dimensionless numbers
\newcommand{\Bo}{\mbox{\textit{Bo}}}
\newcommand{\FvK}{F\"{o}ppl--von K\'{a}rm\'{a}n}
\newcommand{\SL}{\mbox{\textit{S\hspace{-0.07em}\textsmaller[1]{L}}}}


% custom 'check' quantities
\newcommand{\cone}{{\check{1}}}
\newcommand{\ctwo}{{\check{2}}}
\newcommand{\zetaalpha}{\zeta^\calpha}
\newcommand{\zetabeta}{\zeta^\cbeta}
\newcommand{\zetagamma}{\zeta^\cgamma}
\newcommand{\zetaone}{\zeta^\cone}
\newcommand{\zetatwo}{\zeta^\ctwo}


% mesh quantities
\newcommand{\JG}{J^{}_{\Gamma}}
\newcommand{\Jm}{J^{\tm}}
\newcommand{\JO}{J^{}_{\Omega}}
\newcommand{\ptm}{p^{\tm}}
\newcommand{\vm}{v^{\tm}}
\newcommand{\vam}{v^\calpha_{\tm}}
\newcommand{\bmvm}{\bmv^{\tm}}
\newcommand{\zetam}{\zeta^{\tm}}


% solution spaces

\newcommand{\mcth}{\mct_h}
\newcommand{\mcuh}{\mcu_h}

\newcommand{\bmmcu}{\bm{\mcu}}
\newcommand{\bmmcuh}{\bmmcu^{}_{\! h}}
\newcommand{\bmmcv}{\bm{\mcv}}
\newcommand{\bmmcvz}{\bmmcv^{}_{\! 0}}
\newcommand{\bmmcvzh}{\bmmcv^{}_{\! 0, h}}
\newcommand{\bmmcvmz}{\bmmcv^{\tm}_{\! 0}}
\newcommand{\bmmcvmzh}{\bmmcv^{\tm}_{\! 0, h}}
\newcommand{\bmmcvmzv}{\bmmcv^{\tm}_{\! 0, \texttt{v}}}
\newcommand{\bmmcvmzvb}{\bmmcv^{\tm}_{\! 0, \texttt{vb}}}


% finite element variables

\newcommand{\mcgh}{\mcg_h}
\newcommand{\lambdah}{\lambda_h}
\newcommand{\pmh}{\ptm_h}
\newcommand{\bmvh}{\bmv^{}_h}
\newcommand{\bmvmh}{\bmvm_h}
\newcommand{\bmxh}{\bmx^{}_h}

\newcommand{\Nke}{N^{e}_{\mkn k}}
\newcommand{\NJ}{N^{}_{\! J}}
\newcommand{\bmvje}{\bmv^{e}_{\mkn j}}
\newcommand{\bmvke}{\bmv^{e}_{\mkn k}}
\newcommand{\bmvmke}{\bmv^{\tm, e}_{\mkn k}}
\newcommand{\bmvJ}{\bmv^{}_{\! J}}
\newcommand{\bmxke}{\bmx^{e}_{\mkn k}}

\newcommand{\nel}{\texttt{nel}}
\newcommand{\nen}{\texttt{nen}}
\newcommand{\numnp}{\texttt{numnp}}
\newcommand{\poly}{\texttt{poly}}

\newcommand{\mcgA}{\mcg^{\texttt{A}}}
\newcommand{\mcgAv}{\mcg^{\texttt{Av}}}
\newcommand{\mcgAvb}{\mcg^{\texttt{Avb}}}
\newcommand{\mcgE}{\mcg^{\texttt{E}}}
\newcommand{\mcgf}{\mcg_\tf}
\newcommand{\mcgl}{\mcg_\lambda}
\newcommand{\mcgL}{\mcg^{\texttt{L}}}
\newcommand{\mcgm}{\mcg_\tm}
\newcommand{\mcgmA}{\mcg_\tm^{\texttt{A}}}
\newcommand{\mcgmAv}{\mcg_\tm^{\texttt{Av}}}
\newcommand{\mcgmAvb}{\mcg_\tm^{\texttt{Avb}}}
\newcommand{\mcgmE}{\mcg_\tm^{\texttt{E}}}
\newcommand{\mcgp}{\mcg_\tp}
\newcommand{\mcgv}{\mcg_\tv}

\newcommand{\Omegae}{\Omega^e}

\newcommand{\mzero}{[ \bm{0} ]}
\newcommand{\mone}{[ \bm{1} ]}

\newcommand{\mfpt}{[ \mathbff_\tp (t) ]}
\newcommand{\mGe}{[ \mathbfG^e ]}
\newcommand{\mHe}{[ \mathbfH^e ]}
\newcommand{\mK}{[ \mathbfK ]}
\newcommand{\mKt}{[ \mathbfK (t) ]}
\newcommand{\mlambdae}{[ \bmlambda^{\! e} ]}
\newcommand{\mlambdaet}{[ \bmlambda^{\! e} (t) ]}
\newcommand{\mbrlambdaet}{[ \bm{\brlambda}^e (t) ]}
\newcommand{\mNe}{[ \mathbfN^e ]}
\newcommand{\mNep}{[ \mathbfN^e_\tp ]}
\newcommand{\mNeza}{[ \mathbfN^e (\zetaalpha) ]}
\newcommand{\mbrNe}{[ \mathbf{\breve{N}}^e ]}
\newcommand{\mbrNeza}{[ \mathbf{\breve{N}}^e (\zetaalpha) ]}
\newcommand{\mNvece}{[ \mkern-9mu\vec{\mkern9mu\mathbfN^e} ]}
\newcommand{\mNveceza}{[ \mkern-9mu\vec{\mkern9mu\mathbfN^e} (\zetaalpha) ]}
\newcommand{\mNezap}{[ \mathbfN^e (\zetaalphap) ]}
\newcommand{\mpme}{[ \mathbfp^{\tm, e} ]}
\newcommand{\mpmet}{[ \mathbfp^{\tm, e} (t) ]}
\newcommand{\mbrpmet}{[ \mathbf{\brp}^{\tm, e} (t) ]}
\newcommand{\mr}{[ \mathbfr ]}
\newcommand{\mre}{[ \mathbfr^e ]}
\newcommand{\mrel}{[ \mathbfr^e_\lambda ]}
\newcommand{\mremA}{[ \mathbfr^{\texttt{A}, e}_\tm ]}
\newcommand{\mremAv}{[ \mathbfr^{\texttt{Av}, e}_\tm ]}
\newcommand{\mremAvb}{[ \mathbfr^{\texttt{Avb}, e}_\tm ]}
\newcommand{\mremE}{[ \mathbfr^{\texttt{E}, e}_\tm ]}
\newcommand{\mrep}{[ \mathbfr^e_\tp ]}
\newcommand{\mrev}{[ \mathbfr^e_\tv ]}
\newcommand{\mrm}{[ \mathbfr^\tm ]}
\newcommand{\mrmu}{\big[ \mathbfr ( \mbu ) \big]}
\newcommand{\mrmuj}{\big[ \mathbfr ( \mbu_j ) \big]}
\newcommand{\mrmut}{\big[ \mathbfr \big( \mut \big) \big]}
\newcommand{\mrmutj}{\big[ \mathbfr \big( \mut_j \big) \big]}
\newcommand{\mrv}{[ \mathbfr^\tv ]}
\newcommand{\mbu}{[ \mathbfu ]}
\newcommand{\mut}{[ \mathbfu (t) ]}
\newcommand{\mvt}{[ \mathbfv (t) ]}
\newcommand{\mve}{[ \mathbfv^e ]}
\newcommand{\mvet}{[ \mathbfv^e (t) ]}
\newcommand{\mvme}{[ \mathbfv^{\tm, e} ]}
\newcommand{\mvmet}{[ \mathbfv^{\tm, e} (t) ]}
\newcommand{\mxet}{[ \mathbfx^e (t) ]}

\newcommand{\mdeltafp}{[ \delta \mathbff_\tp ]}
\newcommand{\mdeltau}{[ \delta \mathbfu ]}
\newcommand{\mdeltav}{[ \delta \mathbfv ]}
\newcommand{\mdeltavm}{[ \delta \mathbfv^\tm ]}
\newcommand{\mdeltave}{[ \delta \mathbfv^e ]}


% pull force
\newcommand{\mfept}{[ \mathbff^e_\tp (t) ]}
\newcommand{\mdeltafep}{[ \delta \mathbff^e_\tp]}
\newcommand{\mcfp}{\mcf_{\! \tp}}
\newcommand{\mcfpz}{\mcf_{\! \tp, \mk z}}
\newcommand{\mcfeq}{\mcf_{\! \text{eq}}}
\newcommand{\mcfss}{\mcf_{\! \text{ss}}}
\newcommand{\bmmcfp}{\bm{\mcf}_{\! \tp}}
\newcommand{\hnd}{h^*}
\newcommand{\mMep}{[ \mathbfM^e_\tp ]}
\newcommand{\nabland}{\hat{\nabla}}
\newcommand{\Omegaep}{\Omega^e_\tp}
\newcommand{\rnd}{r^*}
\newcommand{\rp}{r^{}_{\mkn \tp}}
\newcommand{\rpnd}{r^{*}_{\mkn \tp}}
\newcommand{\mrvep}{[ \mathbfr^{\tv, e}_\tp ]}
\newcommand{\mrmep}{[ \mathbfr^{\tm, e}_\tp ]}
\newcommand{\mrvnp}{[ \mk \mathbfr^\tv_{\bar{\tp}} \mk ]}
\newcommand{\mrmnp}{[ \mk \mathbfr^\tm_{\bar{\tp}} \mk ]}
\newcommand{\jjbmtp}{\jj{\bmt_\tp}}
\newcommand{\jjbmtpzat}{\jj{\bmt_\tp (\zetaalpha, t)}}
\newcommand{\bmringtp}{\bm{\mathring{t}}_\tp}
\newcommand{\mtept}{[ \mathbf{\mathring{t}}^e_\tp (t) ]}
\newcommand{\mdeltatep}{[ \delta \mathbf{\mathring{t}}^e_\tp ]}
\newcommand{\vp}{v^{}_\tp}
\newcommand{\bmvp}{\bmv^{}_\tp}
\newcommand{\mvept}{[ \mathbfv^e_\tp (t) ]}
\newcommand{\mvmept}{[ \mathbfv^{\tm, e}_\tp (t) ]}
\newcommand{\mvnpt}{[ \mathbfv_{\bar{\tp}} (t) ]}
\newcommand{\mdeltavep}{[ \delta \mathbfv^e_\tp ]}
\newcommand{\mdeltavmep}{[ \delta \mathbfv^{\tm, e}_\tp ]}
\newcommand{\mdeltavnp}{[ \delta \mathbfv_{\bar{\tp}} ]}
\newcommand{\mdeltavmnp}{[ \delta \mathbfv^\tm_{\bar{\tp}} ]}
\newcommand{\zp}{z^{}_\tp}
\newcommand{\zpnd}{z^{*}_{\tp}}
\newcommand{\zetaalphap}{\zeta_\tp \hspace{-3.7pt} {}^{\calpha}}
\newcommand{\zetaonep}{\zeta_\tp \hspace{-3.3pt} {}^{\cone}}
\newcommand{\zetatwop}{\zeta_\tp \hspace{-3.3pt} {}^{\ctwo}}





==> keywords.tex <==
Keywords:
numerical simulation;
finite element analysis;
cell membrane%

